Primordial Rotating Disk Composed of $\geq$15 Dense Star-Forming Clumps at Cosmic Dawn

Early galaxy formation, initiated by the dark matter and gas assembly, evolves through frequent mergers and feedback processes into dynamically hot, chaotic structures. In contrast, dynamically cold, smooth rotating disks have been observed in massive evolved galaxies merely 1.4 billion years after the Big Bang, suggesting rapid morphological and dynamical evolution in the early Universe. Probing this evolution mechanism necessitates studies of young galaxies, yet efforts have been hindered by observational limitations in both sensitivity and spatial resolution. Here we report high-resolution observations of a strongly lensed and quintuply imaged, low-luminosity, young galaxy at $z=6.072$ (dubbed the Cosmic Grapes), 930 million years after the Big Bang. Magnified by gravitational lensing, the galaxy is resolved into at least 15 individual star-forming clumps with effective radii of $r_{\rm e}\simeq$ 10--60 parsec (pc), which dominate $\simeq$ 70\% of the galaxy's total flux. The cool gas emission unveils a smooth, underlying rotating disk characterized by a high rotational-to-random motion ratio and a gravitationally unstable state (Toomre $Q \simeq$ 0.2--0.3), with high surface gas densities comparable to local dusty starbursts with $\simeq10^{3-5}$ $M_{\odot}$/pc$^{2}$. These gas properties suggest that the numerous star-forming clumps are formed through disk instabilities with weak feedback effects. The clumpiness of the Cosmic Grapes significantly exceeds that of galaxies at later epochs and the predictions from current simulations for early galaxies. Our findings shed new light on internal galaxy substructures and their relation to the underlying dynamics and feedback mechanisms at play during their early formation phases, potentially explaining the high abundance of bright galaxies observed in the early Universe and the dark matter core-cusp problem.

==> lineflux_table.tex <==
\scalebox{1.}{
\begin{tabular}{cccc}
\hline
Instrument              & Observed $\lambda$ & Flux density$^{\ddag}$ & reference \\\ 
                        &  [$\mu$m]          & [$\mu$Jy]             &         \\ \hline
 \textit{HST} ACS/F606W & 0.61     & $< 0.07$&   F21  \\
 \textit{HST} ACS/F814W & 0.81     & $0.32\pm0.04$&   F21  \\
 \textit{HST} ACS/F105W & 1.05     & $1.17\pm0.07$ &   F21  \\
 \textit{HST} ACS/F125W & 1.25     & $1.41\pm0.13$ &   F21  \\
 \textit{HST} ACS/F140W & 1.40     & $1.42\pm0.11$ &   F21  \\
 \textit{HST} ACS/F160W & 1.60     & $1.34\pm0.07$ &   F21  \\
 \textit{JWST} NIRCam/F115W & 1.15 & $1.176\pm0.017$ &    This        \\
 \textit{JWST} NIRCam/F150W & 1.50  & $1.521\pm0.008$ &   This        \\
 \textit{JWST} NIRCam/F277W & 2.79  & $2.378\pm0.008$ &   This        \\
 \textit{JWST} NIRCam/F356W & 3.56  & $4.633\pm0.008$ &   This        \\
\textit{JWST} NIRCam/F444W  & 4.42   & $3.130\pm0.010$ &   This        \\
\textit{Herschel} SPIRE 250$\mu$m & 250  & $<$ 15,100    &  S21   \\
\textit{Herschel} SPIRE 350$\mu$m   & 350  & $<$ 16,100  &  S21   \\
\textit{Herschel} SPIRE 500$\mu$m & 500  & $<$ 18,000    &  S21   \\
ALMA Band~8 & 633   & $960\pm520$  &  V24      \\
ALMA Band~7 & 880   & $360\pm50$   &  V24      \\
ALMA Band~7 & 1,005   & $320\pm70$   &  V24      \\
ALMA Band~6 & 1,149   & $200\pm30$   &  V24      \\
ALMA Band~5 & 1,499   & $130\pm30$   &  V24      \\
ALMA Band~3 & 2,790   & $80\pm30$    &  V24      \\ \hline
\end{tabular}
}
